Accelerating Laue Depth Reconstruction Algorithm with CUDA

The Laue diffraction microscopy experiment uses the polychromatic Laue micro-diffraction technique to examine the structure of materials with sub-micron spatial resolution in all three dimensions. During this experiment, local crystallographic orientations, orientation gradients and strains are measured as properties which will be recorded in HDF5 image format. The recorded images will be processed with a depth reconstruction algorithm for future data analysis. But the current depth reconstruction algorithm consumes considerable processing time and might take up to 2 weeks for reconstructing data collected from one single experiment. To improve the depth reconstruction computation speed, we propose a scalable GPU program solution on the depth reconstruction problem in this paper. The test result shows that the running time would be 10 to 20 times faster than the prior CPU design for various size of input data.

==> background.tex <==
In this section, for self containment, we first briefly introduce the
Hungarian method which is often used to solve a matching problem.  We
then use a simple example to illustrate the challenge of reconfiguring
manycore processors for specific applications.   

\subsection{The Hungarian Method for Matching
  Problem}\label{subsec:hm} 
\begin{itemize}
\item what is matching problem
\item what is Hungarian method.  The key, forming the cost matrix
\end{itemize}

\subsection{Application-aware Defect-Spare Core Mapping}
\label{subsec:matching}
\begin{itemize}
\item we can use the example in the paper to show different mapping
  will have different results
\item we have combinatorial number of  different mappings, how to find
  the 'optimal' one?
\end{itemize}

\subsection{Discussion}
\label{subsection:discussion}
\begin{itemize}
\item point out the similarity and difference between job matching
  problem that can be solved by the Hungarian method, and the
  defect-spare core mapping problem
\item point out the goal of the paper, i.e., use the HM solution as an
  approximation to the d-s mapping problem, and investigate the
  performance of the HM in solving the mapping problem
\end{itemize}
%%% Local Variables: 
%%% mode: latex
%%% TeX-master: t
%%% End: 


==> hungarian.tex <==
For self-containment, in this section, we briefly introduce the
assignment problem and the Hungarian method that solves the assignment
problem.

The assignment problem can be stated
as~\cite{kuhn1955hungarian}: there are $n$ workers and $k$
jobs, where $k \leq n$.  Each job can only be assigned to a single
worker.  The time taken by each worker to finish a job is independent and can be different.
The assignment problem is to find a worker to job assignment so that
the total time taken to finish all the jobs is minimized.

The Hungarian method~\cite{kuhn1955hungarian, Jung2009, Gungor2000}
solves the assignment problem in two steps:
\begin{description}
\item[Step 1 :]~  constructs a cost matrix $M_{n \times n}$ where
  $m_{ij}$ is the time cost for worker $i$ ($1\leq i \leq n$) to work
  on job $j$ ($1 \leq j \leq k$). If $n \neq k$, i.e., the numbers of
  workers and the number of jobs are not the same, we augment the
  matrix $M$ to a square one by adding $(n-k)$ number of columns
  filled with zeros.
\item[Step 2 :]~~  uses equivalent matrix reduction to obtain the optimal
  assignment with respect to the cost matrix~\cite{kuhn1955hungarian}
\end{description}

As an example, assume we have three workers $W_1$, $W_2$, and $W_3$,
and three jobs $J_1$, $J_2$, and $J_3$.  It takes $W_1$ 25, 40, and 35
time units to finish job $J_1$, $J_2$, and $J_3$, respectively; for
$W_2$, 40, 60, and 35 and $W_3$, 20, 40, and 25 to finish the three
jobs, respectively.  We have the cost matrix $M_{3 \times 3}$ as:

\[
 M_{3\times3} =
\left[
  \begin{array}{cccc}
    25 & 40 & 35  \\
    40 & 60 & 35  \\
    20 & 40 & 25 \\
  \end{array}
\right]
\]

By iteratively reducing the value in rows and columns, the Hungarian
method is able to get the optimal assignment in $O(n^3)$
time~\cite{James1957}.

% The iterative
% algorithm is briefly summarized in Algorithm~\ref{alg:hm}.

% \begin{algorithm}
%   \caption{\texttt{Hungarian Method ($M_{n\times n}$}, $n$)}
% \label{alg:hm}
% \begin{algorithmic}[1]
%   \STATE Find the minimum value in each row in the cost matrix and
%   subtract it from all the entries in the corresponding row.

%   \STATE Check if there is at lease one zero in each column, if not,
%   subtract the entries of each column with the minimum value in the
%   corresponding column.

%   \STATE Try to draw the minimum number of lines in horizontal or
%   vertical direction to cover all the zeros in the reduced cost
%   matrix.  If the number of lines to cover all the zeros equals to
%   $n$, the final solution is reached.
% %  and we choose the elements from
% %   the original cost matrix as the final assignment, where the values
% %   in the reduced cost matrix for the corresponding elements are zero

%   \STATE Otherwise, find the minimum value in the uncovered part of
%   the reduced matrix, subtract it from the entries in the uncovered
%   rows and then add it to the covered columns. Repeat the step 3) and 4) until the solution found.
% \end{algorithmic}
% \end{algorithm}

For the given cost matrix, the reduced matrix of running the
Hungarian Algorithm is
 \[
  M_{3\times3} =
 \left[
   \begin{array}{cccc}
     0 & \mathbf{0} & 10  \\
     5 & 10 & \mathbf{0}  \\
     \mathbf{0} & 5 & 5 \\
   \end{array}
 \right]
 \]
 \noindent Hence, the optimal assignment is $W_1$, $W_2$, and $W_3$
 for $J_2$, $J_3$, and $J_1$, respectively.

% For the given cost matrix, Algorithm~\ref{alg:hm} provides the optimal
% assignment of $W_1$, $W_2$, and $W_3$ for $J_2$, $J_3$, and $J_1$,
% respectively.


==> motivation.tex <==
In this section, we give a motivating example, define the timing similarity metric and give the problem formulation.



Before giving an example, we first define our application and NoC models.

\begin{definition}[NoC]
  We represent the NoC as an array of physical cores under mesh topology and deterministic XY routing where
  \begin{itemize}
    \item
      $C = \{C_0,C_1,...,C_{M}\}$ are the cores provided by the chip.
      We use $C_{(i)}$ and $C_i$ to denote virtual core and physical core $i$ respectively.
    \item
      $R = \{R_0,R_1,...,R_{N}\}$ are the redundant cores provided by the chip.
    \item
      Virtual Topology $T: C \to C \cup R$ is an injective mapping from virtual cores to
      physical cores.
    \item
      $H_{(i),(j)}^k$ is the number of hops from $C_{(i)}$ to $C_{(j)}$
      along the physical path of the traffic using XY routing algorithm
      for a given virtual topology $T^k$.
  \end{itemize}
  \hfill$\Box$
\end{definition}


\begin{definition}[Mapped Application Task Graph]
A directed acyclic graph $\mathcal{A} = (J,E)$ mapped to a virtual topology where
each vertex $j_{i} \in J$ represents the task mapped to virtual core $C_{(i)}$ and each edge $e_{ij} \in E$ is a data dependency between $j_{i}$ and $j_{j}$. The volume of data sent along the
directed edge $e_{ij}$ is given by $v(e_{ij})$.
\hfill$\Box$
\end{definition}

We make two assumptions regarding the NoC. First, only the cores $C$ become defective. Second, there is no contention in the network. In other words, the NoC bandwidth is sufficiently large. When there is no network contention, the hop count becomes the most important metric for communication times.

\subsection{A Motivating Example}\label{sec:example}

For a given 3x3 NoC with 3 redundant cores as shown in
Fig.\ref{fig:mapping}(c). If, for instance, core $C_4$ is
defective, the remaining defect-free cores form a new \textit{physical
topology}. We can virtualize the defect-free cores and provide
applications a virtual $3\times 3$ mesh topology. There are
several ways to do so, for instance, in
Fig.\ref{fig:mapping}(c), the three redundant cores,
$R_0$, $R_1$, or $R_2$, can be used to replace the defective core
$C_4$, and hence generate three different virtual topologies. Even though applications are given a unified $3\times
3$ mesh, different virtual topologies have different
properties, such as latency and throughput.


For instance, given the application and its initial mapping shown in Fig.\ref{fig:mapping}(a),
consider if the physical core $C_4$ is defective. It can be replaced
by one of the redundant cores $R_0$, $R_1$, or $R_2$. Depending on
which redundant physical core is used, the resulting topologies' hop
count between the virtual cores are different under XY routing(Table~\ref{tab:change}). From the table it is clear that using $R_0$ as the
virtual core $C_4$ is the best choice if the similarity metric is hop count.


Furthermore, if an application is deployed on a topology, the impact on the application of replacing a defective core by different redundant cores also varies.

\begin{figure}[!hbp]
  \centering
  \includegraphics[width=0.45\textwidth]{figure/appmapping.png}
    \caption{Mapping application to cores}
    \label{fig:mapping}
\end{figure}



Generally, for a given application that is mapped to $|J|$ cores
supported by a physical topology with $|R|$ redundant
cores, if among the $|J|$ cores, $p$ ($p \leq \min\{|J|, |R|\}$) cores
become defective, to replace only those defective cores with redundant cores,
we have ${{|R|}\choose{p}} p!$ number of different
choices to form a new virtual topology. Then the question is: which one should we
choose?




\begin{table}[!h]
  \centering
  \begin{tabular}{|p{1.9cm}|p{1.9cm}|p{1cm}|p{1cm}|p{1cm}|}
    \hline
    Traffic Between Virtual Cores & Corresponding Physical Cores & Hop Count\\
    \hline
    $C_{(1)}\rightarrow C_{(4)}$     & $C_1 \rightarrow R_0$ & 2 \\
    \hline
    $C_{(1)}\rightarrow C_{(4)}$     & $C_1 \rightarrow R_1$ & 3 \\
    \hline
    $C_{(1)}\rightarrow C_{(4)}$     & $C_1 \rightarrow R_2$ & 4\\
    \hline
  \end{tabular}
  \caption{Virtualizing different redundant cores for $C_{(4)}$}
  \label{tab:change}
\end{table}

\subsection{Similarity Metric}\label{subsec:metric}

In order to analyze the timing resemblance between a reference topology where there is no defect cores and
a virtual topologies, the timing behavior of a NoC-based manycore
system upon which a specific application is deployed has to be first
defined. As for homogeneous manycore systems, processor speeds are
the same. Hence, on-chip communication becomes a dominant factor that
differentiates various virtual topologies' timing behavior.

We use \textit{traffic time delay} $F_{(i), (j)}$ to quantify the
communication time cost from virtual cores $C_{(i)}$ to $C_{(j)}$.
The formal definition is given below:

\begin{definition}[Traffic Time Delay]
  For a given application and virtual topology $T^k$, the traffic time delay from
  virtual core $C_{(i)}$ to core $C_{(j)}$ is defined as
  \begin{equation}\label{eq:occupancy}
    F_{(i),(j)}^k = v(e_{ij}) + H_{(i),(j)}^k
  \end{equation}

  \hfill$\Box$
\end{definition}

For two different virtual topologies, $T^k$ and
$T^r$, their traffic time delay differences from virtual core
$C_{(i)}$ to $C_{(j)}$ can be calculated by~\eqref{eq:occDiff}
\begin{equation}\label{eq:occDiff}
\Delta_{(i),(j)}^{k, r} =  |F_{(i),(j)}^k - F_{(i),(j)}^r|
\end{equation}
Clearly, the smaller the
traffic time delay differences among \textit{all} virtual core pairs, the higher the
timing similarity among the two topologies. We use normalized
average value ($Ave$) and normalized variation ($Var$) to model the
traffic time delay difference of the entire topology.  Their
definitions are given below:

\begin{definition}
  (\textit{Normalized Average Traffic Time Delay Difference})

  Given an application, a new topology $T^k$ and a reference topology $T^r$, the normalized
  average traffic time delay difference is given by~\eqref{eq:exp}
  \begin{equation}\label{eq:exp}
    Ave_r^k = \displaystyle\frac{
      \displaystyle\sum_{e_{ij}\in E}\Delta_{(i),(j)}^{k,r}
    }{\Psi_r|E|}
  \end{equation}
where $\Psi_r$ is the average traffic time delay of the reference
topology $T^r$ given by~\eqref{eq:ref-ave}.
\begin{equation}\label{eq:ref-ave}
  \Psi_r = \displaystyle\frac{
    \displaystyle \sum_{e_{ij}\in E}F^r_{(i), (j)}}
  {|E|}
\end{equation}

\hfill$\Box$
\end{definition}

\begin{definition}
  (\textit{Normalized Average Variation of Traffic Time Delay Difference})

  Given an application, a new topology $T^k$ and a reference topology $T^r$, the normalized
  variation of traffic time delay difference is given
  by~\eqref{eq:std}
  \begin{equation}\label{eq:std}
    \displaystyle  Var^k_r = \displaystyle\sqrt{\displaystyle\frac{
        \displaystyle\sum_{e_{ij}\in E}(\frac{\Delta_{(i),(j)}^{k,r}}{\Psi_r}-Ave^k_r)^2
      }{|E|} }
\end{equation}
where $\Psi_r$ is given by~\eqref{eq:ref-ave}.

\hfill$\Box$
\end{definition}


Based on the traffic time delay difference between different
topologies, we define virtual topology timing similarity as weighted
sum of normalized average difference and variation. The formal
definition is given below:

\begin{definition}(\textit{Virtual Topology Timing Similarity})

  Given an application, a new topology $T^k$ and a reference topology $T^r$, their timing
  similarity $\chi(T^k_r)$ is defined by~\eqref{eq:similarity}
    \begin{align}\label{eq:similarity}
      \chi(T^k_r)=w_a \times Ave^k_r + w_v \times Var^k_r
     \end{align}
    where $w_a$ and $w_v$ ($w_a +w_v = 1)$ are the weights applied to
    the average difference and average variation, respectively.

    \hfill$\Box$

\end{definition}

\subsection{Problem Formulation}\label{subsec:formulation}

With the similarity metric, we formulate the problem the paper
is to address as follows:

\begin{problem}
  For a given reference topology $T^r$ on which a
  given application $\mathcal{A}$ is deployed, if there are cores used
  by the application $\mathcal{A}$ that become defective, construct a
  virtual topology $T^{opt}$ with defective cores being replaced by redundant cores
  and satisfying the requirement~\eqref{eq:opt}
\begin{align}\label{eq:opt}
  \chi(T^{opt}_r) =\min\{\chi(T^k_r)\}
\end{align}

\hfill$\Box$
\end{problem}

